Fairness in Streaming Submodular Maximization: Algorithms and Hardness

Submodular maximization has become established as the method of choice for the task of selecting representative and diverse summaries of data. However, if datapoints have sensitive attributes such as gender or age, such machine learning algorithms, left unchecked, are known to exhibit bias: under- or over-representation of particular groups. This has made the design of fair machine learning algorithms increasingly important. In this work we address the question: Is it possible to create fair summaries for massive datasets? To this end, we develop the first streaming approximation algorithms for submodular maximization under fairness constraints, for both monotone and non-monotone functions. We validate our findings empirically on exemplar-based clustering, movie recommendation, DPP-based summarization, and maximum coverage in social networks, showing that fairness constraints do not significantly impact utility.

==> 62-video-summarization.tex <==
\subsection{Video Summarization}

In this section, we evaluate the performance of \OurNonMonotone on a video summarization task: Given a stream of video frames, we want to select a diverse subset of frames to concisely represent the video. We use the  Open Video Project (OVP) and the YouTube datasets, which have 50 and 39 videos, respectively \cite{DeAvila2011}. 
A Determinantal Point Process (DPP) is a probability measure over subsets of a ground set of items, used to model diversity. For every $S \subseteq V$, it is defined as $P(S) = \frac{\det(L_S)}{\det(I + L)}$, where $L$ is an $n \times n$ positive semi-definite kernel matrix,  $L_S$ is the $|S| \times |S|$ principal submatrix of $L$ indexed by $S$, and $I$ is the identity matrix. To find the most diverse representative subset, we need to maximize the non-montone submodular function $f(S) = \log\det(L_S)$ \cite{Kulesza2012}. To ensure non-negativity, we add a small diagonal perturbation $\epsilon I$ to $L$ ($\epsilon = 0.1$) and normalize by a constant.

We follow the experimental setup of \cite{gong2014diverse}\footnote{https://github.com/pujols/Video-summarization} to extract frames from videos, and learn a linear kernel matrix $L$.
For a more representative summary, we want the selected frames to be well distributed over the video length. For that, we partition each video into segments of size $T = 20$, and assign frames in each segment to a color.
We set
$\ell_c = \floor*{0.7 \frac{T}{n} k}$
and
$u_c = \ceil*{1.4 \frac{T}{n} k}$, and
 vary $k$ between $5-25\%$ of the total number of frames $n$. 
 The results are shown in \cref{?}. We also evaluate the quality of produced summaries in terms of the F-score, based on $5$ human-generated summaries, as done in \cite{gong2014diverse}, shown in \cref{fig:Fscores}. In this case, adding the fairness constraints actually lead to better solution quality; \OurNonMonotone performs better in terms of F-score, despite the lower objective value.
   \mtodo{we will probably move this figure to the appendix}
   \begin{figure}
   \centering
   \begin{tabular}{cc}
      \includegraphics[trim=25 200 50 200, clip, scale=.25]{Fscore_VideoSummarization_exp_OVP} &       \includegraphics[trim=25 200 50 200, clip, scale=.25]{Fscore_VideoSummarization_exp_YouTube}
   \end{tabular}
   \caption{\label{fig:Fscores} F-scores of summaries generated by \OurNonMonotone and Sample-Streaming.}
   \end{figure}

